A Workload Analysis of NSF's Innovative HPC Resources Using XDMoD

Workload characterization is an integral part of performance analysis of high performance computing (HPC) systems. An understanding of workload properties sheds light on resource utilization and can be used to inform performance optimization both at the software and system configuration levels. It can provide information on how computational science usage modalities are changing that could potentially aid holistic capacity planning for the wider HPC ecosystem. Here, we report on the results of a detailed workload analysis of the portfolio of supercomputers comprising the NSF Innovative HPC program in order to characterize its past and current workload and look for trends to understand the nature of how the broad portfolio of computational science research is being supported and how it is changing over time. The workload analysis also sought to illustrate a wide variety of usage patterns and performance requirements for jobs running on these systems. File system performance, memory utilization and the types of parallelism employed by users (MPI, threads, etc) were also studied for all systems for which job level performance data was available.

==> tables/resource-alloc-used-utilization.tex <==
\begin{table}[H]
\begin{threeparttable}
\centering
\caption{Resource sizes, its portion dedicated to XSEDE, percentage of resource allocated to and used by XSEDE users, node utilization by all users and only by XSEDE users.}
\label{table:resource-alloc-used-utilization}
\small
%\footnotesize
\begin{tabular}{@{}l|rr|R{0.5in}|R{0.4in}R{0.5in}R{0.4in}|R{0.6in}R{0.6in}@{}}
\hline
Resource          & Nodes & Cores  & XSEDE Portion, \% & Allocated, \% of XSEDE & Used, \% of Allocated & Used, \% of Whole\tnote{a} & Node Utilization Total\tnote{s,p}, \% & Node Utilization by XSEDE\tnote{p}, \% \\ \hline

CCT-LSU-SUPERMIC  & 360  & 7200   & 100 & 44  & 62  & 27  & 51 & 28 \\ \hdashline
GATECH-KEENELAND  & 264  & 4224   & 100 & 105\tnote{g} & 76  & 80  &    & 57 \\ \hdashline
NICS-DARTER       & 724  & 11968  & 72\tnote{d}  & 126 & 84  & 106 &    & 53 \\ \hdashline
NICS-KRAKEN       & 9408 & 112896 & 100 & 84  & 103 & 86  &    & \textbf{86} \\ \hdashline
PSC-BLACKLIGHT    & 2    & 4096   & 100 & 81  & 74  & 60  &    & 61 \\ \hdashline
PSC-BRIDGES       & 752  & 21056  & 90  & 74  & 67  & 49  &    & 68 \\ \hdashline
PSC-BRIDGES-GPU   & 48   & 1472   & 100 &     &     &     &    & 50 \\ \hdashline
PSC-BRIDGES-LARGE & 46   & 4512   & 90  &     &     &     &    & 29 \\ \hdashline
PSC-GREENFIELD    & 3    & 360    & 100 & 89  & 26  & 23  &    & 27 \\ \hdashline
PURDUE-STEELE     & 893  & 7144   & 100 & 57  & 74  & 42  &    & 41 \\ \hdashline
SDSC-COMET        & 1944 & 46656  & 100 & 82  & 84  & 68  & \textbf{71} & \textbf{71} \\ \hdashline
SDSC-COMET-GPU    & 72   & 1872   & 100 &     &     &     &    & 93 \\ \hdashline
SDSC-GORDON       & 1024 & 16384  & 85  & 69  & 84  & 58  & 62 & 62 \\ \hdashline
SDSC-TRESTLES     & 324  & 10368  & 70  & 92  & 87  & 80  &    & 67 \\ \hdashline
Stanford-XSTREAM  & 65   & 1300   & 100 & 42\tnote{g}  & 20  & 9   &    & 8  \\ \hdashline
TACC-LONESTAR4    & 1888 & 22656  & 40  & 38  & 81  & 31  & \textbf{74} & 19 \\ \hdashline
TACC-RANGER       & 3936 & 62976  & 100 & 82  & 93  & 76  &    & 75 \\ \hdashline
TACC-STAMPEDE     & 6400 & 102400 & 90  & 73  & 94  & 69  & \textbf{78} & \textbf{69} \\
\hline
\end{tabular}
\begin{tablenotes}
\item[a] Available core hours was calculated for resource production period, some users performed jobs outside of that time.
\item[d] 40\% of NICS-DARTER was dedicated to XSEDE before 2014-05-15 and 90\% afterwards.
\item[s] Calculated using scheduler logs for system where such log was accessible.
\item[p] Node utilization was calculated for each resource during it production period.
\item[g] In this GPU accelerated computing resource allocation was done by GPU hours, for this table it has converted to related node hours.
\end{tablenotes}
\end{threeparttable}
\end{table}

